RaD-Net 2: A causal two-stage repairing and denoising speech enhancement network with knowledge distillation and complex axial self-attention

In real-time speech communication systems, speech signals are often degraded by multiple distortions. Recently, a two-stage Repair-and-Denoising network (RaD-Net) was proposed with superior speech quality improvement in the ICASSP 2024 Speech Signal Improvement (SSI) Challenge. However, failure to use future information and constraint receptive field of convolution layers limit the system's performance. To mitigate these problems, we extend RaD-Net to its upgraded version, RaD-Net 2. Specifically, a causality-based knowledge distillation is introduced in the first stage to use future information in a causal way. We use the non-causal repairing network as the teacher to improve the performance of the causal repairing network. In addition, in the second stage, complex axial self-attention is applied in the denoising network's complex feature encoder/decoder. Experimental results on the ICASSP 2024 SSI Challenge blind test set show that RaD-Net 2 brings 0.10 OVRL DNSMOS improvement compared to RaD-Net.

==> table_edit.tex <==
% \vspace{-0.7em}
\begin{table*}[htbp]
\centering
\small
 \caption{DNSMOS for the repairing network on the ICASSP 2024 SSI Challenge blind test set. ``KD-L" and ``KD-N" denote the knowledge distillation strategy using S1-L as the teacher and the knowledge distillation strategy using S1-N as the teacher. ``S2" and ``S2-A" denote the denoising network and the denoising network with complex ASA.}%%把具体的测试集写一下
 % \vspace{-8pt}
\setlength{\tabcolsep}{0.6mm}
 \label{tab:dnsmos}
  \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccccccccccccccc@{}}
\toprule
    Model & Para.~(M) & SIG & BAK & OVRL & COL & DISC  & LOUD  & NOISE & REVERB & SIG & OVRL       \\ \midrule
    Noisy & - & 3.00 & 3.57 & 2.62 & 3.09 & 3.89 & 3.55 & 3.44 & 3.70 & 3.05 & 2.54       \\ 
    S1 & 2.21 & 3.30 & 4.01 & 3.02 & 3.54 & 4.04 & 4.07 & 4.25 & 4.21 & 3.45 & 3.03    \\
    S1-L & 2.21 & 3.36 & 4.04 & 3.03 & 3.58 & 4.04 & 4.05 & 4.30 & 4.25 & 3.49 & 3.09    \\
    S1-N & 2.21 & 3.43 & 4.05 & 3.16 & 3.73 & 4.19 & 4.14 & 4.34 & 4.27 & 3.72 & 3.32    \\
    S1 with KD-L & 2.21 & 3.31 & 3.99 & 3.03    \\
    S1 with KD-N & 2.21 & 3.36 & 4.02 & 3.09 & 3.63 & 4.06 & 4.05 & 4.28 & 4.20 & 3.54 & 3.10    \\
    S1 + S2 & 4.00 & 3.34 & 4.10 & 3.10 & 3.51 & 4.04 & 4.10 & 4.41 & 4.31 & 3.52 & 3.12    \\
    S1 + S2-A & 3.94 & 3.36 & 4.13 & 3.15 & 3.51 & 4.05 & 4.12 & 4.48 & 4.36 & 3.59 & 3.17    \\
    S1 with KD-N + S2-A & 3.94 & 3.41 & 4.15 & 3.20 & 3.60 & 4.06 & 4.11 & 4.56 & 4.42 & 3.69 & 3.27    \\
\bottomrule
\end{tabular}
}
% \vspace{-2.2em}
\end{table*}
